Equi-Tuning: Group Equivariant Fine-Tuning of Pretrained Models

We introduce equi-tuning, a novel fine-tuning method that transforms (potentially non-equivariant) pretrained models into group equivariant models while incurring minimum $L_2$ loss between the feature representations of the pretrained and the equivariant models. Large pretrained models can be equi-tuned for different groups to satisfy the needs of various downstream tasks. Equi-tuned models benefit from both group equivariance as an inductive bias and semantic priors from pretrained models. We provide applications of equi-tuning on three different tasks: image classification, compositional generalization in language, and fairness in natural language generation (NLG). We also provide a novel group-theoretic definition for fairness in NLG. The effectiveness of this definition is shown by testing it against a standard empirical method of fairness in NLG. We provide experimental results for equi-tuning using a variety of pretrained models: Alexnet, Resnet, VGG, and Densenet for image classification; RNNs, GRUs, and LSTMs for compositional generalization; and GPT2 for fairness in NLG. We test these models on benchmark datasets across all considered tasks to show the generality and effectiveness of the proposed method.

==> gender_equality_word_sets.tex <==
% \usepackage{booktabs}


\begin{table}
\caption{Gender equality word sets taken from \cite{bellamy2019ai} for constructing the $\gE$ set for EquiGPT2.}
\label{tab:gender_equality_words}
\begin{tabular}{ll} 
\toprule
\footnotesize \`{}\`{}\textbf{man}"  & \footnotesize \`{}\`{}\textbf{woman}"  \\ 
\midrule
\vspace{-0.3em}
\tiny male          & \tiny female          \\
\vspace{-0.3em}
\tiny father        & \tiny mother          \\
\vspace{-0.3em}
\tiny him           & \tiny her             \\
\vspace{-0.3em}
\tiny his           & \tiny her             \\
\vspace{-0.3em}
\tiny he            & \tiny she             \\
\vspace{-0.3em}
\tiny himself       & \tiny herself         \\
\vspace{-0.3em}
\tiny king          & \tiny queen           \\
\vspace{-0.3em}
\tiny guy           & \tiny gal             \\
\vspace{-0.3em}
\tiny man           & \tiny woman           \\
\vspace{-0.3em}
\tiny boy           & \tiny girl            \\
\vspace{-0.3em}
\tiny actor         & \tiny actress         \\
\vspace{-0.3em}
\tiny dad           & \tiny mom             \\
\vspace{-0.3em}
\tiny grandson      & \tiny granddaughter   \\
\vspace{-0.3em}
\tiny gentlemen     & \tiny ladies          \\
\vspace{-0.3em}
\tiny gay           & \tiny lesbian         \\
\vspace{-0.3em}
\tiny nephew        & \tiny niece           \\
\vspace{-0.3em}
\tiny salesman      & \tiny saleswoman      \\
\vspace{-0.3em}
\tiny stepfather    & \tiny stepmother      \\
\vspace{-0.3em}
\tiny prince        & \tiny princess        \\
\vspace{-0.3em}
\tiny househusband  & \tiny housewife       \\
\vspace{-0.3em}
\tiny husband       & \tiny wife            \\
\vspace{-0.3em}
\tiny god           & \tiny goddess         \\
\vspace{-0.3em}
\tiny fatherhood    &\tiny  motherhood      \\
\vspace{-0.3em}
\tiny uncle         & \tiny aunt            \\
\vspace{-0.3em}
\tiny patriarch     & \tiny matriarch       \\
\vspace{-0.3em}
\tiny pa            & \tiny ma              \\
\vspace{-0.3em}
\tiny mr            & \tiny miss            \\
\vspace{-0.3em}
\tiny son           & \tiny daughter        \\
\vspace{-0.3em}
\tiny grandpa       & \tiny grandma         \\
\vspace{-0.3em}
\tiny john          & \tiny mary            \\
\vspace{-0.3em}
\tiny boyfriend     & \tiny girlfriend      \\
\vspace{-0.3em}
\tiny brother       & \tiny sister          \\
\vspace{-0.3em}
\tiny adam          &\tiny  ebony           \\
\vspace{-0.3em}
\tiny alan          & \tiny jasmine         \\
\vspace{-0.3em}
\tiny andrew        & \tiny lakisha         \\
\vspace{-0.3em}
\tiny frank         & \tiny latisha         \\
\vspace{-0.3em}
\tiny harry         & \tiny latoya          \\
\vspace{-0.3em}
\tiny jack          & \tiny nichelle        \\
\vspace{-0.3em}
\tiny josh          & \tiny shaniqua        \\
\vspace{-0.3em}
\tiny justin        & \tiny shereen         \\
\vspace{-0.3em}
\tiny roger         & \tiny tanisha         \\
\vspace{-0.3em}
\tiny ryan          & \tiny tia             \\
\vspace{-0.3em}
\tiny alonzo        & \tiny amanda          \\
\vspace{-0.3em}
\tiny alphonse      & \tiny betsy           \\
\vspace{-0.3em}
\tiny darnell       & \tiny courtney        \\
\vspace{-0.3em}
\tiny jamel         & \tiny ellen           \\
\vspace{-0.3em}
\tiny jerome        & \tiny heather         \\
\vspace{-0.3em}
\tiny lamar         & \tiny katie           \\
\vspace{-0.3em}
\tiny leroy         & \tiny kristin         \\
\vspace{-0.3em}
\tiny malik         & \tiny melanie         \\
\vspace{-0.3em}
\tiny terrence      & \tiny nancy           \\
\vspace{-0.3em}
\tiny torrance      & \tiny stephanie       \\
\vspace{-0.3em}
\tiny males         & \tiny female          \\
\vspace{-0.3em}
\tiny fathers       & \tiny mothers         \\
\vspace{-0.3em}
\tiny kings         & \tiny queens          \\
\vspace{-0.3em}
\tiny guys          & \tiny gals            \\
\vspace{-0.3em}
\tiny men           & \tiny women           \\
\vspace{-0.3em}
\tiny boys          & \tiny girls           \\
\vspace{-0.3em}
\tiny actors        & \tiny actresses       \\
\vspace{-0.3em}
\tiny dads          & \tiny moms            \\
\vspace{-0.3em}
\tiny grandsons     & \tiny granddaughters  \\
\vspace{-0.3em}
\tiny gays          & \tiny lesbians        \\
\vspace{-0.3em}
\tiny nephews       & \tiny nieces          \\
\vspace{-0.3em}
\tiny salesmen      & \tiny saleswomen      \\
\vspace{-0.3em}
\tiny stepfathers   & \tiny stepmothers     \\
\vspace{-0.3em}
\tiny princes       & \tiny princesses      \\
\vspace{-0.3em}
\tiny househusbands & \tiny housewives      \\
\vspace{-0.3em}
\tiny husbands      & \tiny wives           \\
\vspace{-0.3em}
\tiny gods          & \tiny goddesses       \\
\vspace{-0.3em}
\tiny uncles        & \tiny aunts           \\
\vspace{-0.3em}
\tiny patriarchs    & \tiny matriarchs      \\
\vspace{-0.3em}
\tiny sons          & \tiny daughters       \\
\vspace{-0.3em}
\tiny grandpas      & \tiny grandmas        \\
\vspace{-0.3em}
\tiny boyfriends    & \tiny girlfriends     \\
\vspace{-0.3em}
\tiny brothers      & \tiny sisters         \\
\tiny gentleman     & \tiny lady           \\
\bottomrule
\end{tabular}
\vspace{-100pt}
\end{table}
